Multi-Document Scientific Summarization from a Knowledge Graph-Centric View

Multi-Document Scientific Summarization (MDSS) aims to produce coherent and concise summaries for clusters of topic-relevant scientific papers. This task requires precise understanding of paper content and accurate modeling of cross-paper relationships. Knowledge graphs convey compact and interpretable structured information for documents, which makes them ideal for content modeling and relationship modeling. In this paper, we present KGSum, an MDSS model centred on knowledge graphs during both the encoding and decoding process. Specifically, in the encoding process, two graph-based modules are proposed to incorporate knowledge graph information into paper encoding, while in the decoding process, we propose a two-stage decoder by first generating knowledge graph information of summary in the form of descriptive sentences, followed by generating the final summary. Empirical results show that the proposed architecture brings substantial improvements over baselines on the Multi-Xscience dataset.

==> data/temp.tex <==
\section{Experiments}
\subsection{Dataset}
We conduct experiments with the recently released Multi-Xscience dataset~\citep{lu2020multi}, which is the first large scale and open MDSS dataset. It contains 30,369 instances for training, 5,066 for validation and 5,093 for test. On average, each source paper cluster contains 4.42 papers and 778.08 words, and each gold summary contains 116.44 words.

\subsection{Implementation Details}
We set our model parameters based on preliminary experiments on the validation set. We prune the vocabulary to 50K. The number of encoder layer $L$ and the number of decoder layer $L_2$ are both 6. We set the dimension of word embeddings and hidden size to 256, feed-forward size to 1,024. We set 8 heads for multi-head attention. For graph updater and entity-sentence updater, we set the number of iterations to 2. We set dropout rate to 0.1 and label smoothing~\citep{szegedy2016rethinking} factor to 0.1. We use Adam optimizer with learning rate $\alpha=0.02$, $\beta_1=0.9$, $\beta_2=0.998$; we also apply learning rate warmup over the first 8000 steps,  and decay as in~\citep{vaswani2017attention}. The batch size is set to 8. $\lambda$ and $\eta$ are both set to 1.0. The model is trained on 1 GPU (NVIDIA Tesla V100, 32G) for 100,000 steps. We select the top-3 best checkpoints based on performance on the validation set and report averaged results on the test set.

For backbone decoding, we use gready search with the minimal generation length 100, while for summary decoding, we use beam search with beam  size 5 and the minimal generation length is 110 consistent with~\citep{lu2020multi}. The length penalty factor is set to 0.4.

\subsection{Metrics and Baselines}
We use ROUGE $F_1$~\citep{lin2004rouge} to evaluate the summarization quality. Following previous work, we report unigram and bigram overlap (ROUGE-1 and ROUGE-2) as a mean of assessing informativeness and the longest common subsequence (ROUGE-L) as a means of assessing fluency. We compare our model with several typical baselines and several baselines proposed recently. 

\textbf{LexRank}~\citep{erkan2004lexrank} and \textbf{TextRank}~\citep{mihalcea2004textrank} are two unsupervised graph based extractive summarization models. \textbf{HeterSumGraph}~\cite{wang2020heterogeneous} is a heterogeneous graph-based extractive model with semantic nodes of different granularity.  \textbf{HiMAP}~\citep{fabbri2019multi} expands the pointer-generator network~\citep{see2017get} into a hierarchical network and integrates an MMR module. \textbf{HierSumm}~\citep{liu2019hierarchical} is a
Transformer based model with an attention mechanism
to share information cross-document for abstractive
multi-document summarization. \textbf{MGSum}~\citep{jin2020multi} is a multi-granularity interaction network for abstractive
multi-document summarization. We also consider evaluating on single document summarization models by concatenating multiple papers into a long sequence.
\textbf{Pointer-Generator}~\citep{see2017get} is an RNN based model with an attention mechanism and allows the system to copy words from the source via pointing for abstractive summarization.
\textbf{BertABS}~\citep{liu2019text} uses a pretrained BERT~\citep{devlin2019bert} as the encoder for abstractive summarization. We also report the performance of BertABS with an encoder (\textbf{SciBertABS}) pretrained on scientific articles.
\textbf{BART}~\citep{lewis2020bart} is a pretrained text generation model.

\subsection{Automatic Evaluation}

\begin{table}[tb]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
    \resizebox{\columnwidth}{!}{
    \hfill
    \small
     \renewcommand\arraystretch{1.1}
    \begin{tabular}{l|lll}
    %\toprule
    \hline
    \textbf{Model} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
    \multicolumn{4}{l}{\emph{Extractive}}\\ \cline{1-4}
    LexRank & 30.19& 5.53& 26.19\\
    TextRank & 31.51& 5.83& 26.58\\
    HeterSumGraph & 31.36& 5.82& 27.41\\
    Ext-Oracle & 38.45 & 9.93 & 27.11 \\\hline
    \multicolumn{4}{l}{\emph{Abstractive}}\\\hline
    Hiersumm & 30.02& 5.04& 27.6\\
    HiMAP & 31.66& 5.91& 28.43\\
    BertABS & 31.56& 5.02& 28.05\\
    MGSum & 32.28& 6.49& 28.32\\
    BART & 32.83& 6.36& 26.61\\
    SciBertABS & 32.12& 5.59& 29.01\\
    Pointer-Generator & 34.11& 6.76& 30.63\\
    \hline
    KGSum & \textbf{35.77}& \textbf{7.51}&  \textbf{31.43} \\
    %\bottomrule
    \hline
    \end{tabular}
    }
    \caption{ROUGE F1 evaluation results on the test set of Multi-Xscience.}
    \label{table1}
\end{table}

Table~\ref{table1} summarizes the evaluation results on the Multi-Xscience dataset. As can be seen, our abstractive model outperforms any other models, achieving scores of 35.77, 7.51, 31.43 on the three ROUGE metrics. Our model surpasses other models by a remarkable large margin (at least improving 1.66\%, 0.75\% and 0.80\%). The result demonstrates that our model can generate more informative and more coherent summary, indicating
the effectiveness of our proposed knowledge graph-centric encoder and decoder framework.

We also find that abstractive models generally outperform extractive models, indicating that the gold summary of Multi-Xscience tends to use novel words to summarize papers. To some extent, it shows that MDSS task is more suitable to be solved by abstractive approaches than extractive ones.

\begin{table*}[htb]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\hline
\renewcommand\arraystretch{1.1}
\multirow{2}*{\textbf{Models}} & \multicolumn{5}{c|}{\textbf{Informativeness}} & \multicolumn{5}{c}{\textbf{Fluency}} \\     
	%\hline
	\cline{2-11}
	 & \tabincell{c}{\textbf{1st}} & \tabincell{c}{\textbf{2nd}} &\tabincell{c}{\textbf{3rd}} & \tabincell{c}{\textbf{4th}} & \tabincell{c}{\textbf{rating}} &  \tabincell{c}{\textbf{1st}} & \tabincell{c}{\textbf{2nd}} &\tabincell{c}{\textbf{3rd}} & \tabincell{c}{\textbf{4th}} & \tabincell{c}{\textbf{rating}}\\
\hline
MGSum & - & -& -& - &- &- &- &- &-& -\\
Pointer-Generator & - & -& -& - &- &- &- &- &-& - \\
GraphSum & - & -& -& - &- &- &- &- &-& -\\
KGSum & - & -& -& - &- &- &- &- &-& -\\
\hline
\end{tabular}
}
\caption{Human evaluation of generated summary. 1st is the best and 4th is the worst. The larger rating denotes better summary quality. * indicates the overall ratings of the corresponding model are significantly (by Welch’s t-test with p < 0:05)
outperformed by our model. The inter-annotator agreement score (Cohen Kappa) is \_, which indicates substantial agreement
between annotators. }
\label {table461}
\end{table*}

\subsection{Human Evaluation}
In addition to automatic evaluation, we also access system performance by human evaluation. We randomly select 30 test instances from the Multi-Xscience test set, and invite 3 graduate students as annotators to evaluate the outputs of different models independently. Annotators assess the overall quality of summaries by ranking them considering the following criteria:: (1) \emph{Informativeness}: does the summary convey important facts of the input papers? (2) \emph{Fluency}: is the summary fluent and grammatical? Annotators were asked to ranking all systems from 1 (best) to 4 (worst). All systems get score 2, 1, -1, -2 for ranking 1, 2, 3, 4 respectively. The rating of each system is computed by averaging the scores on all test instances.

The result is shown in table~\ref{table461}.

\subsection{Model Analysis}
For a thorough understanding of KGSum, we conduct several experiments on Multi-Xscience test set.

\begin{table}[tb]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
    \resizebox{\columnwidth}{!}{
    \hfill
    \small
     \renewcommand\arraystretch{1.1}
    \begin{tabular}{l|lll}
    %\toprule
    \hline
    \textbf{Model} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
    \textbf{KGSum} & \textbf{35.77}& \textbf{7.51}&  \textbf{31.43}\\
    - BG & 35.34& 7.28& 30.91\\
    - BG - RAKE & 35.17& 7.18& 30.75\\
    - BG - RAKE - GU & 34.97 & 7.08 & 30.63 \\
    - BG - RAKE - GU - ESU & 34.79 & 6.90 & 30.36 \\
    \hline
    \end{tabular}
    }
    \caption{Ablation studies on Multi-Xscience test set. We remove various modules and explore their influence on our model. '-' means the removal operation from KGSum. The last row (-BG-RAKE-GU-ESU) is the clean baseline without any module we proposed. }
    \label{table2}
\end{table}

\paragraph{Ablation Study} Firstly, we perform an ablation study to validate the effectiveness of individual components. Here, \textbf{BG} stands for backbone generator, \textbf{RAKE} refers to the RAKE algorithm that measures entity salience, \textbf{GU} stands for graph updater, \textbf{ESU} stands for entity-sentence updater. We remove BG, RAKE, GU, ESU one by one in order from decoder to encoder. The result is illustrated in table~\ref{table2}. We could find that the GU and ESU module in the encoder can effectively encode knowledge graph information and utilize knowledge graph to enable better information flowing between text nodes, which is conducive to content modeling and relationship modeling. Using RAKE to measure entity salience also benefits a lot for graph context computation when decoding. Further, the BG module also brings significant improvement, indicating our proposed two-stage decoder with backbone generator is effective in generating summary under the guidance of knowledge graph.

\paragraph{Recall of Entity Words} In order to intuitively display the impact of knowledge graph, we investigate recall of entity words in the generated summary. First we define \textbf{Entity Words} (EW) as words in the text that are recognized as entity by SciIE tools, while \textbf{Context Words} (CW) are defined as words other than EW. Recall of EW is calculated as:
\begin{equation}
\small
Recal{l_{EW}} = \frac{{\sum\limits_{S \in \{ Ref\} } {\sum\limits_{{N_{EW}} \in S} {Coun{t_{match}}({N_{EW}})} } }}{{\sum\limits_{S \in \{ Ref\} } {\sum\limits_{{N_{EW}} \in S} {Count({N_{EW}})} } }}
\end{equation}

\begin{table}[tb]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
    \resizebox{\columnwidth}{!}{
    \hfill
    \small
     \renewcommand\arraystretch{1.1}
    \begin{tabular}{l|ll}
    %\toprule
    \hline
    \textbf{Model} & \textbf{Recall-EW} & \textbf{Recall-CW}\\ \hline
    \emph{Upper Bound} & 45.3 & 50.25 \\\hline
    MGSum & 20.45& 36.54\\
    Pointer-Generator & 24.96 & 38.17 \\
    Baseline & 24.4 & 38.44 \\
    \textbf{KGSum} & \textbf{26.17}& \textbf{39.35}\\
    \hline
    \end{tabular}
    }
    \caption{Recall of EW and CW on the test set of Multi-Xscience.}
    \label{table3}
\end{table}

where ${\{ Ref\} }$ denotes the gold summaries, ${Coun{t_{match}}({N_{EW}})}$ denotes the number of overlapped EW in the gold summaries and  the generated summaries. ${Count({N_{EW}})}$ denotes the number of EW in the gold summaries. Recall of CW is defined in a similar manner. The result of recall of EW and CW is shown in Table~\ref{table3}. The table shows that our KGSum can generate more accurate entity words, thus  conveying more important information, thanks to the knowledge graph. However, it's worth noting that the upper bound of recall of EW and CW are 45.3\% and 50.25\%, suggesting that there is still a long way to go to generate a better summary. 

\begin{table}[tb]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
    \resizebox{\columnwidth}{!}{
    \hfill
    \small
     \renewcommand\arraystretch{1.1}
    \begin{tabular}{l|lll}
    %\toprule
    \hline
    \textbf{Backbone Variants} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
    Ent & 35.61 & 7.43 & 31.24 \\
    Ent+Type & 35.67 & 7.42 & 31.29 \\
    \textbf{Ent+Type+Rel} & \textbf{35.77}& \textbf{7.51}&  \textbf{31.43}\\
    \hline
    \end{tabular}
    }
    \caption{Analysis of the impact of different backbone contents on summarization. \textbf{Ent} refers to using only entities to construct backbone. \textbf{Ent+Type} refers to using entities and types, \textbf{Ent+Type+Rel} refers to using entities, types and relations. }
    \label{table4}
\end{table}

\paragraph{Influence of Backbone Contents} We also conduct experiments to analyze the impact of different backbone contents on summarization. We consider the following three variants: (1) only entities (Ent), (2) entities + types (Ent+Type), (3) entities + types + relations (Ent+Type+Rel), to construct the backbone using the same strategy in section~\ref{bg}. Result in Table~\ref{table4} demonstrates MDSS task can benefit from 
different components of knowledge graph, including entities, types and relations. 



==> data/temp2.tex <==
\subsection{Encoder}
Given a set of papers as input, we first establish vector representations for words, entities and sentences. Let ${w_{i,j}}$ be the $j$-th word of the sentence $s_{i}$, each word ${w_{i,j}}$ is converted into vector representation ${ e_{i,j}}$ by learned emebddings. We also assign positional encoding to indicate the position of ${w_{i,j}}$ and two positions are considered, namely sentence index $i$ and word index $j$. Then we concatenate the position embeddings $PE_i$, $PE_j$ to obtain the final position embedding $p_{i,j}$. The definition of postional encoding is consistent with the Transformer~\cite{vaswani2017attention}. The final word representation is obtained by simply add ${\hat e_{i,j}}$ and $p_{i,j}$. 
\begin{eqnarray}
{p_{i,j}} = [P{E_i};P{E_j}]\\
h_{{w_{i,j}}}^0 = {{ e}_{i,j}} + {p_{i,j}}
\end{eqnarray}

The encoder follows a standard transformer architecture ~\cite{vaswani2017attention}. It takes $h_{{w_{i,j}}}^0$ (for all tokens) as input. For the $l$-th transformer layer, we perform multi-head self-attention across the word representation $h_{{w_{i,j}}}^{l-1}$ in the sentence $s_i$ to compute the contextual word representation $h_{{w_{i,j}}}^{l}$:

\begin{eqnarray}
\hat h_{{w_{i,j}}}^{l - 1} = {\rm{LayerNorm}}(h_{{w_{i,j}}}^{l - 1} + {\rm{MHAtt(}}h_{{w_{i,j}}}^{l - 1}{\rm{))}}\\
h_{{w_{i,j}}}^l = {\rm{LayerNorm}}(\hat h_{{w_{i,j}}}^{l - 1} + {\rm{FFN(}}\hat h_{{w_{i,j}}}^{l - 1}{\rm{)}})
\end{eqnarray}

where LayerNorm is the layer normalization proposed in \citet{ba2016layer}; MHAtt means the multi-head attention module proposed in ~\citet{vaswani2017attention} and FFN is a two-layer feed-forward network with ReLU as hidden activation function. 

After obtaining contextual word representation, we follow \citet{liu2019hierarchical} to apply a multi-head pooling operation to get sentence representation $h_{{s_i}}^l$. The multi-head pooling mechanism calculates the weight distributions over tokens, allowing the model to flexibly encode sentences in different representational subspaces by different heads.
\begin{eqnarray}
h_{{s_i}}^l = {\rm{MHPool(}}h_{{w_{i,1}}}^l{\rm{,}}h_{{w_{i,2}}}^l{\rm{,}}...{\rm{)}}
\end{eqnarray}

We perform the same encoding process as the sentence encoder to obtain the entity representation $h_{{e_i}}^l$ for entity $e_i$.

\begin{table*}[htb]
\centering
%\resizebox{0.9\textwidth}{!}{
{
\begin{tabular}{l|ccccc|ccccc}
\hline
%\renewcommand\arraystretch{1.1}
\multirow{2}*{\textbf{Models}} & \multicolumn{5}{c|}{\textbf{Informativeness}} & \multicolumn{5}{c}{\textbf{Fluency}} \\     
	%\hline
	\cline{2-11}
	 & \tabincell{c}{\textbf{1st}} & \tabincell{c}{\textbf{2nd}} &\tabincell{c}{\textbf{3rd}} & \tabincell{c}{\textbf{4th}} & \tabincell{c}{\textbf{rating}} &  \tabincell{c}{\textbf{1st}} & \tabincell{c}{\textbf{2nd}} &\tabincell{c}{\textbf{3rd}} & \tabincell{c}{\textbf{4th}} & \tabincell{c}{\textbf{rating}}\\
\hline
MGSum & - & -& -& - &- &- &- &- &-& -\\
Pointer-Generator & - & -& -& - &- &- &- &- &-& - \\
GraphSum & - & -& -& - &- &- &- &- &-& -\\
KGSum & - & -& -& - &- &- &- &- &-& -\\
\hline
\end{tabular}
}
\caption{Human evaluation of generated summary. 1st is the best and 4th is the worst. The larger rating denotes better summary quality. * indicates the overall ratings of the corresponding model are significantly (by Welch’s t-test with p < 0.05)
outperformed by our model. The inter-annotator agreement score (Cohen Kappa) is \_, which indicates substantial agreement
between annotators. }
\label {table461}
\end{table*}

Multi-document scientific summarization (MDSS) can be classified into different tasks according to different application scenarios, such as scientific topic summarization or survey generation when given a scientific topic~\citep{mohammad2009using,jha2015surveyor,yang2017keyphraseds}, or related work generation when given a target paper and its references~\citep{hoang2010towards,hu2014automatic,wang2018neural,chen2021capturing}.

\begin{equation}
\small
Recal{l_{EW}} = \frac{{\sum\limits_{S \in \{ Ref\} } {\sum\limits_{{N_{EW}} \in S} {Coun{t_{match}}({N_{EW}})} } }}{{\sum\limits_{S \in \{ Ref\} } {\sum\limits_{{N_{EW}} \in S} {Count({N_{EW}})} } }}
\end{equation}
